Bayesian Covariance Estimation for Multi-group Matrix-variate Data

Multi-group covariance estimation for matrix-variate data with small within group sample sizes is a key part of many data analysis tasks in modern applications. To obtain accurate group-specific covariance estimates, shrinkage estimation methods which shrink an unstructured, group-specific covariance either across groups towards a pooled covariance or within each group towards a Kronecker structure have been developed. However, in many applications, it is unclear which approach will result in more accurate covariance estimates. In this article, we present a hierarchical prior distribution which flexibly allows for both types of shrinkage. The prior linearly combines shrinkage across groups towards a shared pooled covariance and shrinkage within groups towards a group-specific Kronecker covariance. We illustrate the utility of the proposed prior in speech recognition and an analysis of chemical exposure data.

==> MiscFiles/latex_macros.tex <==
%Math commands
\newcommand\E{\mathbb{E}}
\newcommand\Fs{\mathcal{F}}
\newcommand\Cs{\mathcal{C}}
\newcommand\Ps{\mathcal{P}}
\newcommand\Ls{\mathcal{L}}
\newcommand\As{\mathcal{A}}
\newcommand\Bs{\mathcal{B}}
\newcommand\Ss{\mathcal{S}}
\newcommand\Gs{\mathcal{G}}
\newcommand\Hs{\mathcal{H}}
\newcommand\Es{\mathcal{E}}
\newcommand\Ts{\mathcal{T}}
\newcommand\Ns{\mathcal{N}}
\newcommand\Us{\mathcal{U}}
\newcommand\Os{\mathcal{O}}
\newcommand\Vs{\mathcal{V}}
\newcommand\Ds{\mathcal{D}}

\newcommand{\Tau}{\mathrm{T}}


\newcommand\reals{\mathbb{R}}
\newcommand\naturals{\mathbb{N}}
\newcommand\diadics{\mathbb{Q}_2}
\newcommand\rationals{\mathbb{Q}}
\usepackage{bbm}
\newcommand\indicator{\mathbbm{1}}

\newcommand\siga{\sigma\text{-algebra}}
\newcommand\ls{\lambda\text{-system}}
\newcommand\ps{\pi\text{-system}}

\newcommand\variance{\sigma^2}

\newcommand\he{\hat{e}}
\newcommand\hbeta{\hat{\beta}}
\newcommand\htheta{\hat{\theta}}
\newcommand\hY{\hat{Y}}
\newcommand\hy{\hat{y}}
\newcommand\hmu{\hat{\mu}}
\newcommand\hvariance{\hat{\sigma^2}}
\newcommand\hp{\hat{p}}
\newcommand\hbs{\hat{\Sigma}}
\newcommand\hbp{\hat{\Psi}}
\newcommand\hbl{\hat{\Lambda}}

\newcommand\bs{\Sigma}
\newcommand\bl{\Lambda}
\newcommand\bo{\Omega}
\newcommand\bg{\Gamma}
\newcommand\bp{\Psi}

\newcommand\barY{\bar{Y}}
\newcommand\bary{\bar{y}}

\newcommand\ystar{Y_*}
\newcommand\hystar{\hat{Y_*}}
\newcommand\xstar{X_*}
\newcommand\xstart{X_*^T}
\newcommand\mustar{\mu_*}
\newcommand\epsstar{\epsilon_*}

\newcommand\xinv{X^{-1}}

\newcommand\indep{\perp \!\!\! \perp}

% all one vectors
\newcommand\onen{\mathbf{1}_n}
\newcommand\onent{\mathbf{1}_n^T}
\newcommand\onep{\mathbf{1}_p}
\newcommand\onept{\mathbf{1}_p^T}
\newcommand\one{\mathbf{1}}

% bold parameters
\newcommand\thetabf{{\boldsymbol{\theta}}}
\newcommand\Ybf{\boldsymbol{Y}}
\newcommand\ybf{\boldsymbol{y}}
\newcommand\Xbf{\boldsymbol{X}}
\newcommand\xbf{\boldsymbol{x}}
\newcommand\wbf{\boldsymbol{w}}
\newcommand{\nbf}{\boldsymbol{n}}
\newcommand{\mubf}{\boldsymbol{\mu}}
\newcommand{\alphabf}{\boldsymbol{\alpha}}
\newcommand{\lambdabf}{\boldsymbol{\lambda}}

\newcommand\norm[1]{||#1||^2}

\newcommand\kron{\;\otimes\;}

\newcommand\zbold{\boldsymbol{z}}
\newcommand\hbold{\boldsymbol{h}}

% distributed in special ways
\newcommand\myeq{\stackrel{\mathclap{\normalfont\mbox{s}}}{~}}
\newcommand\distind{\stackrel{ind}{\sim}}
\newcommand\distiid{\stackrel{iid}{\sim}}
\newcommand\distexch{\stackrel{exch}{\sim}}
\newcommand\equalind{\stackrel{D}{=}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% Not math commands:
\newcommand\KI{\textbf{Key Idea: }}


